The giant outburst of EXO 2030+375 II: Broadband spectroscopy and evolution

In 2021, the high-mass X-ray binary EXO 2030+375 underwent a giant X-ray outburst, the first since 2006, that reached a peak flux of ${\sim}600\,\mathrm{mCrab}$ (3-50\,keV). The goal of this work is to study the spectral evolution over the course of the outburst, search for possible cyclotron resonance scattering features (CRSFs), and to associate spectral components with the emission pattern of the accretion column. We used broadband spectra taken with the Nuclear Spectroscopic Telescope Array (NuSTAR), the Neutron Star Interior Composition Explorer (NICER), and Chandra near the peak and during the decline phase of the outburst. We describe the data with established empirical continuum models and perform pulse-phase-resolved spectroscopy. We compare the spectral evolution with pulse phase using a proposed geometrical emission model. We find a significant spectral hardening toward lower luminosity, a behavior that is expected for super-critical sources. The continuum shape and evolution cannot be described by a simple power-law model with exponential cutoff; it requires additional absorption or emission components. We can confirm the presence of a narrow absorption feature at ${\sim}10\,\mathrm{keV}$ in both NuSTAR observations. The absence of harmonics puts into question the interpretation of this feature as a CRSF. The empirical spectral components cannot be directly associated with identified emission components from the accretion column.

==> CRSF-limits.tex <==
 \begin{table}
 \centering
 \caption{Centroid optical depth $\tau$ of absorption features at previously reported CRSF energies. Line widths have been fixed during fitting. }
 \label{tab:crsf_test}
    \begin{tabular}{cccc}
    \hline\hline
    Energy & Width & Obs.~I & Obs.~II\\
    \hline
    10\,keV & 2.5\,keV & $0.049^{+0.003}_{-0.004}$ & $0.038\pm0.008$ \\
    36\,keV & 1.0\,keV & $0.048\pm0.020$ & $\le0.025$\\
    63\,keV & 5.0\,keV &$\le0.025$ & $\le0.048$ \\
      \hline\hline
      \end{tabular}
  \end{table}
      

==> table-hetg-par.tex <==
\begin{table}
 \centering
 \caption{Best-fit parameters for the \chandra/HETG spectrum of \exo. All line widths were fixed to 10\,eV.}
 \label{tab:hetg_bestfit}
    \begin{tabular}{lc}
      \hline\hline
     parameter & value \\
     \hline
     $N_\mathrm{H}$\tablefootmark{a} & $2.26^{+0.06}_{-0.07}$ \\
     $F_\mathrm{PL}$\tablefootmark{b} & $4.49\pm0.03$ \\
     $\Gamma$ & $1.05^{+0.06}_{-0.05}$ \\
     $kT_\mathrm{BB}$\tablefootmark{c} & $0.63^{+0.04}_{-0.06}$ \\
     $F_\mathrm{BB}$\tablefootmark{b} & $0.28\pm0.02$ \\
     $E_\mathrm{{\ion{Si}{xiv}\,Ly}\alpha}$\tablefootmark{c} & $2.41^\dagger$\\
     $A_\mathrm{{\ion{Si}{xiv}\,Ly}\alpha}$\tablefootmark{d} & $0.74^{+0.29}_{-0.30}$\\
     $E_\mathrm{{Fe\,K}\alpha}$\tablefootmark{c} & $6.40^\dagger$\\
     $A_\mathrm{{Fe\,K}\alpha}$\tablefootmark{d} & $0.27^{+0.22}_{-0.18}$\\
     $E_\mathrm{{\ion{Fe}{xxv}\,He}\alpha}$\tablefootmark{c} & $6.70^\dagger$\\
     $A_\mathrm{{\ion{Fe}{xxv}\,He}\alpha}$\tablefootmark{d} & $0.42^{+0.25}_{-0.24}$\\
     $E_\mathrm{{\ion{Fe}{xxvi}\,Ly}\alpha}$\tablefootmark{c} & $6.97^\dagger$\\
     $A_\mathrm{{\ion{Fe}{xxvi}\,Ly}\alpha}$\tablefootmark{d} & $<0.38$\\
         \hline\hline
      \end{tabular}
        \tablefoot{
        \tablefoottext{a}{In $10^{22}\,\mathrm{cm}^{-2}$.}
       \tablefoottext{b}{Unabsorbed 0.1--10\,keV flux in $10^{-9}\,\mathrm{erg}\,\mathrm{s}^{-1}\,
        \mathrm{cm}^{-2}$.}
        \tablefoottext{c}{In keV.}
        \tablefoottext{d}{Photon flux in $10^{-3}\,\mathrm{phs}\,\mathrm{cm}^{-2}\,\mathrm{s}^{-1}$.}
           }
  \end{table}

 %  tbabs*(powerlaw+bbody+gaussian(3)+gaussian(2)+gaussian(1)+gaussian(4))
 % idx  param             tie-to  freeze         value         min         max
 %  2  powerlaw(1).norm       0     0        0.3328372   0.3005308   0.3740909  
 %  4  bbody(1).norm          0     0      0.003668841  0.002690836  0.004639304  
 
 

==> table-phaseavg_par.tex <==
 \begin{table}
 \centering
 \caption{Best-fit parameters for the phase-averaged spectrum of \nustar Obs.~I and II. A partial covering absorber is not required in Obs.~II.}
 \label{tab:phasavg_bestfit}
    \begin{tabular}{lcc}
      \hline\hline
      parameter & Obs.\ I & Obs.\ II \\
      \hline
      $c_\mathrm{FPMB}$ & $0.9878^{+0.0018}_{-0.0017}$ &  $0.9988^{+0.0030}_{-0.0029}$ \\
      $c_\mathrm{XTI}$ &  $1.032\pm0.006$ & $0.939\pm0.005$ \\
       $N_{\mathrm{H},1}$\tablefootmark{a} & $3.9^{+0.8}_{-0.6}$
                          & $2.64\pm0.03$ \\
      $N_{\mathrm{H},2}$\tablefootmark{a} & $2.15^{+0.25}_{-0.47}$ & --- \\
      pcf &  $0.71^{+0.18}_{-0.16}$ &  --- \\
      $kT_\mathrm{BB}$\tablefootmark{b} & $0.472^{+0.036}_{-0.028}$ & $2.44\pm0.04$ \\
      $F_\mathrm{BB}$\tablefootmark{c} &  $0.58^{+0.18}_{-0.13}$ & $0.47\pm{0.03}$  \\
      $\Gamma$ & $1.114^{+0.011}_{-0.012}$ & $1.019\pm0.014$  \\
      $E_\mathrm{fold}$\tablefootmark{b} & $18.22^{+0.17}_{-0.18}$ &  $19.3\pm0.4$ \\
      $F_\mathrm{PL}$\tablefootmark{d} & $15.51^{+0.08}_{-0.07}$ & $4.81^{+0.04}_{-0.05}$ \\
      $A_\mathrm{Fe}$\tablefootmark{e} &  $6.7\pm0.4$ &  $1.91^{+0.23}_{-0.21}$  \\
      $E_\mathrm{Fe}$\tablefootmark{b} &  $6.594^{+0.023}_{-0.019}$ & $6.54\pm0.05$ \\
      $\sigma_\mathrm{Fe}$\tablefootmark{b} & $0.277^{+0.018}_{-0.017}$ &
                                                         $0.33\pm0.05$
      \\
      $E_\mathrm{10\,keV}$\tablefootmark{b} & $10.23^{+0.13}_{-0.15}$ & $9.4\pm0.4$ \\
      $\sigma_\mathrm{10\,keV}$\tablefootmark{b} & $2.58^{+0.29}_{-0.23}$ & $1.8^{+0.6}_{-0.4}$\\
      $d_\mathrm{10\,keV}$\tablefootmark{b} &  $0.32^{+0.06}_{-0.05}$ &  $0.13^{+0.10}_{-0.05}$ \\
      $\mathcal{L}$\tablefootmark{f} & $1.1\times10^{37}$ &  $3.6\times10^{36}$\\
      $\mathrm{GS}_\mathrm{FPMA}$\tablefootmark{g} &  $-29^{+15}_{-19}$ &  $-80^{+29}_{-20}$ \\
      $\mathrm{GS}_\mathrm{FPMB}$\tablefootmark{g} & $-37^{+14}_{-18}$ & $-75^{+27}_{-25}$ \\ 
      $\mathrm{GS}_\mathrm{XTI}$\tablefootmark{g} & $-9\pm4$ & $1.2^{+2.8}_{-2.7}$\\
      \hline\hline
      \end{tabular}
      \tablefoot{
        \tablefoottext{a}{In $10^{22}\,\mathrm{cm}^{-2}$.}
        \tablefoottext{b}{In keV.}
        \tablefoottext{c}{Unabsorbed 1--10\,keV flux in $10^{-9}\,\mathrm{erg}\,\mathrm{s}^{-1}\,
        \mathrm{cm}^{-2}$.}
        \tablefoottext{d}{Unabsorbed 3--50\,keV flux in $10^{-9}\,\mathrm{erg}\,\mathrm{s}^{-1}\,
        \mathrm{cm}^{-2}$.}
        \tablefoottext{e}{Photon flux in $10^{-3}\,\mathrm{phs}\,\mathrm{cm}^{-2}\,\mathrm{s}^{-1}$.}
         \tablefoottext{f}{3--50\,keV luminosity in $\mathrm{erg}\,\mathrm{s}^{-1}$ for a distance of 2.4\,kpc.}   
        \tablefoottext{g}{Additive gainshift in eV.}
      }
  \end{table}
